A new method to determine $H_0$ from cosmological energy-density measurements

We introduce a new method for measuring the Hubble parameter from low-redshift large-scale observations that is independent of the comoving sound horizon. The method uses the baryon-to-photon ratio determined by the primordial deuterium abundance, together with Big Bang Nucleosynthesis (BBN) calculations and the present-day CMB temperature to determine the physical baryon density $\Omega_b h^2$. The baryon fraction $\Omega_b/\Omega_m$ is measured using the relative amplitude of the baryonic signature in galaxy clustering measured by the Baryon Oscillation Spectroscopic Survey, scaling the physical baryon density to the physical matter density. The physical density $\Omega_mh^2$ is then compared with the geometrical density $\Omega_m$ from Alcock-Paczynski measurements from Baryon Acoustic Oscillations (BAO) and voids, to give $H_0$. Including type Ia supernovae and uncalibrated BAO, we measure $H_0 = 67.1^{+6.3}_{-5.3}$ km s$^{-1}$ Mpc$^{-1}$. We find similar results when varying analysis choices, such as measuring the baryon signature from the reconstructed correlation function, or excluding supernovae or voids. This measurement is currently consistent with both the distance-ladder and CMB $H_0$ determinations, but near-future large-scale structure surveys will obtain 3--4$\times$ tighter constraints.

==> PRL_summary.tex <==
The Hubble parameter defines our place in the Universe. It controls how fast the Universe is expanding and can be directly linked to the time elapsed since the Big Bang. There are two current methods to determine the Hubble parameter - one uses stars of known brightness in nearby galaxies, and one uses the overall properties of the Universe as measured by the cosmic microwave background. They give different results at a statistically significant level, meeting the ``5-$\sigma$'' standard that is usually taken as indicative of a discovery.
A scientific paper published today in Physical Review Letters  presents a new method for measuring the Hubble parameter. This is based on energy densities in the Universe, rather than distances. As space expands the density of matter decreases, so measuring densities can therefore lead to a measurement of the expansion rate.
To measure the density of material in the universe, the authors had to include both the material that we can easily observe - because it interacts with light - and the dark matter that does not. To do this, they looked at how galaxies are distributed in the Universe. They were able to decompose the pattern into two components - one for the material we can see, and one for the material we cannot. The amplitude of each component lets us measure the ratio of the different types of material in the Universe.
While the measurements made do not solve the tension between other measurements, the method will soon be applied to forthcoming data that will revolutionise the field. The Dark Energy Spectroscopic Instrument and Euclid projects, both which are underway, will use this method to measure the Hubble parameter and will achieve constraints that will differentiate between previous measurement differences. 
